"Violation of my body:" Perceptions of AI-generated non-consensual (intimate) imagery

AI technology has enabled the creation of deepfakes: hyper-realistic synthetic media. We surveyed 315 individuals in the U.S. on their views regarding the hypothetical non-consensual creation of deepfakes depicting them, including deepfakes portraying sexual acts. Respondents indicated strong opposition to creating and, even more so, sharing non-consensually created synthetic content, especially if that content depicts a sexual act. However, seeking out such content appeared more acceptable to some respondents. Attitudes around acceptability varied further based on the hypothetical creator's relationship to the participant, the respondent's gender and their attitudes towards sexual consent. This study provides initial insight into public perspectives of a growing threat and highlights the need for further research to inform social norms as well as ongoing policy conversations and technical developments in generative AI.

==> visuals/vignetteFactors.tex <==
\begin{table*}[]
\renewcommand{\arraystretch}{1.2}
\centering
\footnotesize
\begin{tabular}{lll}
\toprule
\textbf{Factor} & \textbf{Description} & \textbf{Levels} \\
\midrule
\textsf{creator} 
    & The individual utilizing generative AI to create the media & an intimate partner, a stranger \\
\midrule
\textsf{action} 
    & The action being performed by the participant in the synthetic media & performing a sexual act, playing a sport, saying something \\
\midrule
\textsf{intent} 
    & The creator's motivation for generating the synthetic media & harming you, entertainment, sexual pleasure \\
\bottomrule
\end{tabular}
\caption{The factors and their levels that we varied and presented in the synthetic media vignettes.}
\label{tab:vignette-factors}
\end{table*}
